MAIRA-1: A specialised large multimodal model for radiology report generation

We present a radiology-specific multimodal model for the task for generating radiological reports from chest X-rays (CXRs). Our work builds on the idea that large language model(s) can be equipped with multimodal capabilities through alignment with pre-trained vision encoders. On natural images, this has been shown to allow multimodal models to gain image understanding and description capabilities. Our proposed model (MAIRA-1) leverages a CXR-specific image encoder in conjunction with a fine-tuned large language model based on Vicuna-7B, and text-based data augmentation, to produce reports with state-of-the-art quality. In particular, MAIRA-1 significantly improves on the radiologist-aligned RadCliQ metric and across all lexical metrics considered. Manual review of model outputs demonstrates promising fluency and accuracy of generated reports while uncovering failure modes not captured by existing evaluation practices. More information and resources can be found on the project website: https://aka.ms/maira.

==> tables/without_finetuning.tex <==
\begin{table}[htb]
\centering
\caption{Comparison of \maira{} against zero-shot baselines from pre-existing models (i.e.~not trained specifically for radiology report generation). LLaVA-1.0 and LLaVA-1.5 are general-domain models and LLaVA-Med was continually trained from LLaVA-1.0 on biomedical data.
\WIP{As expected, the base models---which were trained on diverse instruction-tuning datasets for generalist capabilities---are entirely unable to perform the report generation task with basic prompting. This highlights the need for training specialised models for such a complex and nuanced application.}
\TODO{[Daniel] Please double-check}
}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{} l l|c c c|c}\toprule
    Category & Metric & LLaVA-1.0 & LLaVA-Med & LLaVA-1.5 & \maira{} \\
    \midrule
    Lexical & 
    ROUGE-L & 
        13.2 {\scriptsize \textcolor{gray}{[13.1, 13.4]}} & %
        13.3 {\scriptsize \textcolor{gray}{ [13.1, 13.4]}} & %
        14.0 {\scriptsize \textcolor{gray}{[13.9, 14.1]}} & %
        28.9 {\scriptsize \textcolor{gray}{[28.4, 29.4]}} \\
    & BLEU-4 & 
         3.3 {\scriptsize \textcolor{gray}{[3.2, 3.3]}} & %
         0.6 {\scriptsize \textcolor{gray}{ [0.5, 0.7]}} &  %
         1.3 {\scriptsize \textcolor{gray}{[1.2, 1.4]}} & %
        14.2 {\scriptsize \textcolor{gray}{[13.7, 14.7]}} \\
    & METEOR & 
        21.7 {\scriptsize \textcolor{gray}{[21.4, 21.8]}} & %
        14.4 {\scriptsize \textcolor{gray}{ [14.3, 14.6]}} &  %
        17.4 {\scriptsize \textcolor{gray}{[17.3, 17.5]}} & %
        33.3 {\scriptsize \textcolor{gray}{[32.8, 33.8]}}\\
    \midrule
    Clinical & 
    RadGraph-F1 & 
         1.8 {\scriptsize \textcolor{gray}{[1.7, 1.9]}} & %
         2.4 {\scriptsize \textcolor{gray}{[2.3, 2.5]}} & %
         2.0 {\scriptsize \textcolor{gray}{[1.9, 2.1]}} & %
        24.3 {\scriptsize \textcolor{gray}{[23.7, 24.8]}}\\
    & RG\textsubscript{ER} & 
         2.9 {\scriptsize \textcolor{gray}{[2.7, 3.0]}} & %
         4.1 {\scriptsize \textcolor{gray}{[3.8, 4.2]}} &  %
         3.3 {\scriptsize \textcolor{gray}{[3.1, 3.4]}} & %
        29.6 {\scriptsize \textcolor{gray}{[29.0, 30.2]}}\\
    & CheXbert vector & 
        17.7 {\scriptsize \textcolor{gray}{[17.2, 18.3]}} & %
        13.3 {\scriptsize \textcolor{gray}{[12.7, 13.8]}} & %
        19.2 {\scriptsize \textcolor{gray}{[18.7, 19.7]}} & %
        44.0 {\scriptsize \textcolor{gray}{[43.1, 44.9]}} \\
    & RadCliQ ($\downarrow$) & 
        4.75 {\scriptsize \textcolor{gray}{[4.74, 4.77]}} & %
        4.78 {\scriptsize \textcolor{gray}{[4.77, 4.79]}} &  %
        4.77 {\scriptsize \textcolor{gray}{[4.76, 4.78]}} & %
        3.10 {\scriptsize \textcolor{gray}{[3.07, 3.14]}}\\
\cmidrule{2-6}
    & Macro-F1-14 & 
         5.9 {\scriptsize \textcolor{gray}{[5.4, 6.5]}} & %
         7.7 {\scriptsize \textcolor{gray}{ [7.1, 8.4]}} & %
         6.6 {\scriptsize \textcolor{gray}{[6.2, 7.1]}} & %
        38.6 {\scriptsize \textcolor{gray}{[37.1, 40.1]}} \\
    & Micro-F1-14 & 
        14.1 {\scriptsize \textcolor{gray}{[13.1, 15.2]}} & %
        15.8 {\scriptsize \textcolor{gray}{ [14.7, 16.8]}} & %
        19.4 {\scriptsize \textcolor{gray}{[18.3, 20.7]}} & %
        55.7 {\scriptsize \textcolor{gray}{[54.7, 56.8]}} \\
    & Macro-F1-5 & 
         7.2 {\scriptsize \textcolor{gray}{[6.5, 7.9]}} & %
        5.5 {\scriptsize \textcolor{gray}{ [4.6, 6.5]}} & %
         9.5 {\scriptsize \textcolor{gray}{[8.9, 10.0]}} & %
        47.7 {\scriptsize \textcolor{gray}{[45.6, 49.5]}} \\
    & Micro-F1-5 &
        15.0 {\scriptsize \textcolor{gray}{[13.4, 16.5]}} & %
        7.5 {\scriptsize \textcolor{gray}{ [6.2, 8.9]}} & %
        24.1 {\scriptsize \textcolor{gray}{[22.5, 25.7]}} & %
        56.0 {\scriptsize \textcolor{gray}{[54.5, 57.5]}} \\
    \bottomrule
\end{tabular}
\label{tab:without_finetuning}
\end{table}








